On the Concept Trustworthiness in Concept Bottleneck Models

Concept Bottleneck Models (CBMs), which break down the reasoning process into the input-to-concept mapping and the concept-to-label prediction, have garnered significant attention due to their remarkable interpretability achieved by the interpretable concept bottleneck. However, despite the transparency of the concept-to-label prediction, the mapping from the input to the intermediate concept remains a black box, giving rise to concerns about the trustworthiness of the learned concepts (i.e., these concepts may be predicted based on spurious cues). The issue of concept untrustworthiness greatly hampers the interpretability of CBMs, thereby hindering their further advancement. To conduct a comprehensive analysis on this issue, in this study we establish a benchmark to assess the trustworthiness of concepts in CBMs. A pioneering metric, referred to as concept trustworthiness score, is proposed to gauge whether the concepts are derived from relevant regions. Additionally, an enhanced CBM is introduced, enabling concept predictions to be made specifically from distinct parts of the feature map, thereby facilitating the exploration of their related regions. Besides, we introduce three modules, namely the cross-layer alignment (CLA) module, the cross-image alignment (CIA) module, and the prediction alignment (PA) module, to further enhance the concept trustworthiness within the elaborated CBM. The experiments on five datasets across ten architectures demonstrate that without using any concept localization annotations during training, our model improves the concept trustworthiness by a large margin, meanwhile achieving superior accuracy to the state-of-the-arts. Our code is available at https://github.com/hqhQAQ/ProtoCBM.

==> tables/ablation_CLA_CIA.tex <==
\begin{table}[ht]
\renewcommand\arraystretch{1}
\small
\centering
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{c *4{c}}
  \toprule
\textbf{\small Method} & \textbf{\small ResNet34} & \textbf{\small ResNet152} & \textbf{\small Dense161} & \textbf{\small DeiT-S} \\

\midrule

{\small w/o CLA \& CIA} & 12.13 & 6.76 & 11.16 & 10.91 \\
{\small \bf w/ CLA \& CIA} & {\bf 44.36} & {\bf 55.95} & {\bf 40.32} & {\bf 58.44} \\

  \bottomrule
  \end{tabular}}
%   }
\caption{The CLA \& CIA modules significantly improve the alignment between deep and shallow feature maps under spatial transformation. w/ \& w/o denote without \& with.}
\label{tab:ablation_CLA_CIA}

\end{table}

==> tables/ablation_PA.tex <==
\begin{table}[ht]
\renewcommand\arraystretch{1}
\small
\centering
\setlength{\tabcolsep}{0.68mm}{
\begin{tabular}{c *3{c}}
  \toprule
\textbf{\small Method} & \textbf{\small Head - Head($\uparrow$)} & \textbf{\small Head - Leg($\downarrow$)} & \textbf{\small Leg - Leg($\uparrow$)} \\

\midrule

{\small w/o $\mathcal{L}_{\rm grp}$ \& $\mathcal{L}_{\rm div}$} & 32.34 & 37.63 & 36.07  \\
{\small w/ $\mathcal{L}_{\rm grp}$ } & 56.74 & 34.92 & 43.15 \\
{\small w/ $\mathcal{L}_{\rm grp}$ \& $\mathcal{L}_{\rm div}$ } & \textbf{93.59} & \textbf{20.55} & \textbf{56.91} \\

  \bottomrule
  \end{tabular}}
%   }
\caption{The PA module remarkably increases the IoU between the localization regions of the concepts with the same related regions~(Head - Head, Leg - Leg), and separates the concepts with different related regions~(Head - Leg). Note that $\uparrow$ denotes higher is better, while $\downarrow$ is the opposite.}
\label{tab:ablation_PA}

\end{table}
